Large-scale Charging of Electric Vehicles: A Multi-Armed Bandit Approach

The successful launch of electric vehicles (EVs) depends critically on the availability of convenient and economic charging facilities. The problem of scheduling of large-scale charging of EVs by a service provider is considered. A Markov decision process model is introduced in which EVs arrive randomly at a charging facility with random demand and completion deadlines. The service provider faces random charging costs, convex non-completion penalties, and a peak power constraint that limits the maximum number of simultaneous activation of EV chargers. Formulated as a restless multi-armed bandit problem, the EV charging problem is shown to be indexable. A closed-form expression of the Whittle's index is obtained for the case when the charging costs are constant. The Whittle's index policy, however, is not optimal in general. An enhancement of the Whittle's index policy based on spatial interchange according to the less laxity and longer processing time principle is presented. The proposed policy outperforms existing charging algorithms, especially when the charging costs are time varying.

==> LLLP_v3.tex <==
%In \cite{Xu&Pan:2012CDC}, the authors proposed

The LLLP principle is a priority rule for the scheduling
of charging multiple EVs, which is defined as follows.
\begin{Def}[The LLLP Principle]
Consider chargers (arms) $i$ and $j$ at time $t$. We say $j$ dominates $i$ ($j\succeq i$),
if $j$ has less laxity and longer remaining processing time, \ie $B_j[t] \ge B_i[t]$ and $L_j[t]\le L_j[t]$, with at least one of the inequalities strictly holds.
\end{Def}



LLLP defines a partial order over the EVs' states such that the EV with less laxity and longer remaining charging demand should be given priority.
In \cite{Xu&Pan:2012CDC}, the authors applied an interchange argument to show that LLLP could improve the performance of any given policy along every sample path,
 and further, there exists an optimal stationary policy that follows the LLLP principle under mild conditions.

The LLLP interchange can be easily implemented to improve any given policy $\pi$. As illustrated in Fig.~\ref{fig:LLLP}, suppose that at time $t$, EV $j$ has less laxity and longer remaining charging demand than EV $i$ ($j\succeq i$), and that the policy $\pi$ charges $i$ but not $j$.
An LLLP interchange improved policy $\tilde{\pi}$ charges $j$ but not $i$ at time $t$.
\textcolor[rgb]{1.00,0.00,0.00}{\emph{May not needed since we do not change back:} Let $t' \in [t+1,\min\{d_i,d_j\}]$ denote the time period at which
 $\pi$ charges $j$ but not $i$ for the first time; at time $t'$, $\tilde{\pi}$ charges $i$ but not $j$.
If such a period $t'$ does not exist, then the interchanging policy $\tilde{\pi}$ will take the same action as the
original policy $\pi$ after time $t$.}


The LLLP principle results in many smaller unfinished jobs rather than fewer and larger unfinished jobs.
 As a result, it always improves the profit performance under time-varying charging costs and convex non-completion penalty functions.
 We wiil apply the LLLP principle to improve the Whittle's index policy.





\begin{figure}
\centering
\psfrag{i}{{\footnotesize $i$}}
\psfrag{Bi}{{\footnotesize $B_i[t]$}}
\psfrag{Bj}{{\footnotesize $B_j[t]$}}
\psfrag{Ti}{{\footnotesize $T_i[t]$}}
\psfrag{Tj}{{\footnotesize $T_j[t]$}}
\psfrag{j}{{\footnotesize $j$}}
\psfrag{pi}{{\footnotesize$\pi$}}
\psfrag{pitilde}{{\footnotesize$\tilde{\pi}$}}
\psfrag{active}{{\footnotesize active}}
\psfrag{passive}{{\footnotesize passive}}
\psfrag{t}{{\small $t$}}
\psfrag{tau}{{\small $\tau$}}
\psfrag{time}{{\small time}}
  % Requires \usepackage{graphicx}
  \includegraphics[width=0.5\textwidth]{figs/LLLP2.eps}
  \caption{The LLLP interchange}
  \label{fig:LLLP}
\end{figure}


